An Empirical Study of Partial Deduction for miniKanren

We study conjunctive partial deduction, an advanced specialization technique aimed at improving the performance of logic programs, in the context of relational programming language miniKanren. We identify a number of issues, caused by miniKanren peculiarities, and describe a novel approach to specialization based on partial deduction and supercompilation. The results of the evaluation demonstrate successful specialization of relational interpreters. Although the project is at an early stage, we consider it as the first step towards an efficient optimization framework for miniKanren.

==> eptcsdata.tex <==
\providecommand{\firstpage}{73}
\providecommand{\publicationstatus}{Alexei Lisitsa and Andrei Nemytykh (Eds.): 9th International Workshop\\ on Verification and Program Transformation (VPT 2021)\\
EPTCS 341, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.341.5}{10.4204/EPTCS.341.5}}
\pdfoutput=1

